Complete Description of Matching Polytopes with One Linearized Quadratic Term for Bipartite Graphs

We consider, for complete bipartite graphs, the convex hulls of characteristic vectors of all matchings, extended by a binary entry indicating whether the matching contains two specific edges. These polytopes are associated to the quadratic matching problems with a single linearized quadratic term. We provide a complete irredundant inequality description, which settles a conjecture by Klein (Ph.D. thesis, TU Dortmund, 2015). In addition, we also derive facetness and separation results for the polytopes. The completeness proof is based on a geometric relationship to a matching polytope of a nonbipartite graph. Using standard techniques, we finally extend the result to capacitated b-matchings.

==> tikz-quadratic-bipartite-matching-graphs.tex <==
\piDeclareString{job}{}
\piDeclareBool{down support graph}{false}
\piDeclareBool{up support graph}{false}
\piDeclareBool{down gadget}{false}
\piDeclareBool{up gadget}{false}
\piDeclareBool{up cycles}{false}
\piDeclareBool{color}{false}
\piDeclareBool{debug}{false}

\piParse % Parses all given options

% Debugging code

\piIfBool{down support graph}{
  \def\boundingbox{(0,-0.3) rectangle (5,6)};
}{}
\piIfBool{up support graph}{
  \def\boundingbox{(0,-0.3) rectangle (5,6)};
}{}
\piIfBool{down gadget}{
  \def\boundingbox{(0,-0.3) rectangle (8,5)};
}{}
\piIfBool{up gadget}{
  \def\boundingbox{(1,-0.3) rectangle (7,5)};
}{}
\piIfBool{up cycles}{
  \def\boundingbox{(1,-0.3) rectangle (7.5,5)};
}{}

\draw[clip,use as bounding box,draw=none] \boundingbox;
\piIfBool{debug}{
  \draw[step=.5cm,help lines] (-11,-20) grid (11,20);
  \draw[draw=red,thick] \boundingbox;
}{}

% Drawing code

\def\graphNodesA{}
\def\graphNodesB{}
\def\graphNormalEdges{}
\def\graphSpecialEdges{}

\piIfBool{down support graph}{
  \def\graphNodesA{1/1.5/5, 2/1.5/4,3/1.5/2.5,4/1.5/1.5,5/1.5/0.5}
  \def\graphNodesB{1/3.5/5, 2/3.5/4,3/3.5/2.5,4/3.5/1.5,5/3.5/0.5}
  \def\graphNormalEdges{%
    a-1/b-2, a-1/b-3, a-1/b-4, a-1/b-5,
    a-2/b-1, a-2/b-3, a-2/b-4, a-2/b-5,
    a-3/b-1, a-3/b-2, a-3/b-3, a-3/b-4, a-3/b-5,
    a-4/b-1, a-4/b-2, a-4/b-3, a-4/b-4, a-4/b-5,
    a-5/b-1, a-5/b-2, a-5/b-3, a-5/b-4, a-5/b-5}
  \def\graphSpecialEdges{a-1/b-1, a-2/b-2}
}{}

\piIfBool{up support graph}{
  \def\graphNodesA{1/1.5/5, 2/1.5/4,3/1.5/2.5,4/1.5/1.5,5/1.5/0.5}
  \def\graphNodesB{1/3.5/5, 2/3.5/4,3/3.5/2.5,4/3.5/1.5,5/3.5/0.5}
  \def\graphNormalEdges{%
    a-1/b-2, a-2/b-1,
    a-1/b-3, a-1/b-4, a-1/b-5,
    a-2/b-3, a-2/b-4, a-2/b-5,
    a-3/b-1, a-3/b-2, a-3/b-3, a-3/b-4, a-3/b-5,
    a-4/b-1, a-4/b-2, a-4/b-3, a-4/b-4, a-4/b-5,
    a-5/b-1, a-5/b-2, a-5/b-3, a-5/b-4, a-5/b-5}
  \def\graphSpecialEdges{a-1/b-1, a-2/b-2}
}{}

\piIfBool{down gadget}{
  \def\graphNodesA{1/2/4, 2/2/1, 3/2/-5}
  \def\graphNodesB{1/6/4, 2/6/1, 3/6/-5}
  \def\graphNormalEdges{%
    a-1/b-2, a-1/b-3,
    a-2/b-1, a-2/b-3,
    a-3/b-1, a-3/b-2}
}{}

\piIfBool{up gadget}{
  \def\graphNodesA{1/2/4, 2/2/1, 3/2/-5}
  \def\graphNodesB{1/6/4, 2/6/1, 3/6/-5}
  \def\graphNormalEdges{%
    a-1/b-2, a-1/b-3,
    a-2/b-1, a-2/b-3,
    a-3/b-1, a-3/b-2}
}{}

% Graph

\tikzset{
  graphNodeStyle/.style={draw=black, thick, fill=black!20!white, circle, inner sep=0, minimum size=4mm},
  graphNormalEdgeStyle/.style={draw=black, ultra thin},
  graphSpecialEdgeStyle/.style={draw=black, ultra thick, dashed},
}

\piIfBool{color}{
  \tikzset{
    graphGreenEdgeStyle/.style={draw=green!80!black},
    graphRedEdgeStyle/.style={draw=red},
  }
}{
  \tikzset{
    graphGreenEdgeStyle/.style={dotted},
    graphRedEdgeStyle/.style={dashed},
  }
}

\foreach \i/\x/\y in \graphNodesA {
  \coordinate (a-\i) at (\x,\y);
}

\foreach \i/\x/\y in \graphNodesB {
  \coordinate (b-\i) at (\x,\y);
}

\piIfBool{down support graph}{
  \draw[thick,draw=black!50!white,fill=black!10!white, rounded corners] 
    (1.1,5.4) -- (1.9,5.4) -- (1.9,2.9) -- (3.9,2.9) -- (3.9,1.1) -- (3.1,1.1) -- (3.1,2.1) -- (1.1,2.1) -- cycle;
}{}

\piIfBool{up support graph}{
  \draw[thick,draw=black!50!white,fill=black!10!white, rounded corners] 
    (1.1,5.4) -- (2.9,5.4) -- (2.9,4.8) -- (3.3,4.4)  -- (3.9,4.4) -- (3.9,1.1) -- (1.1,1.1) -- (1.1,2.9) -- (2.5,2.9) -- (2.5,4.0) -- (2.0,4.6) -- (1.1,4.6) -- cycle;
}{}

\foreach \i/\x/\y in \graphNodesA {
  \node[graphNodeStyle] (a-\i) at (a-\i) {};
  \node[left=2mm of a-\i] {$u_{\i}$};
}

\foreach \i/\x/\y in \graphNodesB {
  \node[graphNodeStyle] (b-\i) at (b-\i) {};
  \node[right=2mm of b-\i] {$w_{\i}$};
}

\foreach \u/\v in \graphNormalEdges {
  \draw[graphNormalEdgeStyle] (\u) -- (\v);
}

\foreach \u/\v in \graphSpecialEdges {
  \draw[graphSpecialEdgeStyle] (\u) -- (\v);
}

\piIfBool{down support graph}{
  \node at (2.5,5.25) {$e_1$};
  \node at (2.5,4.25) {$e_2$};
}{}

\piIfBool{up support graph}{
  \node at (2.6,4.75) {$e_1$};
  \node at (2.6,4.25) {$e_2$};
}{}

\piIfBool{down gadget}{
  \draw[very thick, graphRedEdgeStyle] (a-1) -- (b-1);
  \draw[very thick, graphRedEdgeStyle] (a-2) -- (b-2);
  \draw[very thick, graphGreenEdgeStyle] (a-1) -- (a-2);
  \draw[very thick, graphGreenEdgeStyle] (b-1) -- (b-2);

  \node at (4,4.25) {$\hat{x}_{e_1} - \hat{y}$};
  \node at (4,0.75) {$\hat{x}_{e_2} - \hat{y}$};
  \node[anchor=east] at (2,2.5) {$\hat{y}$};
  \node[anchor=west] at (6,2.5) {$\hat{y}$};
}{}

\piIfBool{up gadget}{
  \node[graphNodeStyle] (u) at (4,3.2) {};
  \node[graphNodeStyle] (v) at (4,1.8) {};
  \node[above right=0mm of u] {$a$};
  \node[below right=0mm of v] {$b$};

  \draw[very thick, graphRedEdgeStyle] (a-1) to[bend angle=15,bend left] (b-1);
  \draw[very thick, graphRedEdgeStyle] (a-2) to[bend angle=15,bend right] (b-2);
  \draw[very thick, graphRedEdgeStyle] (u) -- (v);
  \draw[very thick, graphGreenEdgeStyle] (a-1) -- (u) -- (b-2);
  \draw[very thick, graphGreenEdgeStyle] (a-2) -- (v) -- (b-1);

  \node[scale=0.8] at (4,4.6) {$\frac{1}{2}\hat{y}$};
  \node[scale=0.8] at (4,0.4) {$\frac{1}{2}\hat{y}$};
  \node[anchor=east,scale=0.8] at (3.85,2.5) {$1 - \hat{x}_{e_1} - \hat{x}_{e_2} + \hat{y}$};
  \node[anchor=west,scale=0.8] at (2.8,3.8) {$\hat{x}_{e_1} - \frac{1}{2}\hat{y}$};
  \node[anchor=west,scale=0.8] at (2.8,1.2) {$\hat{x}_{e_2} - \frac{1}{2}\hat{y}$};
  \node[anchor=west,scale=0.8] at (5.2,3.05) {$\hat{x}_{e_1} - \frac{1}{2}\hat{y}$};
  \node[anchor=west,scale=0.8] at (5.2,1.95) {$\hat{x}_{e_2} - \frac{1}{2}\hat{y}$};
}{}

\piIfBool{up cycles}{
  % First cycle.

  \node[graphNodeStyle] (a-1) at (1.5,4+0.5) {};
  \node[graphNodeStyle] (b-1) at (5.5,4+0.5) {};
  \node[graphNodeStyle] (u-1) at (3.5,3.2+0.5) {};
  \node[graphNodeStyle] (v-1) at (3.5,1.8+0.5) {};
  
  \draw[very thick, graphRedEdgeStyle] (a-1) -- (b-1);
  \draw[very thick, graphRedEdgeStyle] (u-1) -- (v-1);
  \draw[very thick, graphGreenEdgeStyle] (a-1) -- (u-1);
  \draw[very thick, graphGreenEdgeStyle] (b-1) -- (v-1);
  
  \node at (2.5,3) {$C_1$};

  % Second cycle.
  
  \node[graphNodeStyle] (a-2) at (1.5+1.5,1-1) {};
  \node[graphNodeStyle] (b-2) at (5.5+1.5,1-1) {};
  \node[graphNodeStyle] (u-2) at (3.5+1.5,3.2-1) {};
  \node[graphNodeStyle] (v-2) at (3.5+1.5,1.8-1) {};
  
  \draw[very thick, graphRedEdgeStyle] (a-2) -- (b-2);
  \draw[very thick, graphRedEdgeStyle] (u-2) -- (v-2);
  \draw[very thick, graphGreenEdgeStyle] (a-2) -- (v-2);
  \draw[very thick, graphGreenEdgeStyle] (b-2) -- (u-2);

  \node at (6.5,1.5) {$C_2$};
}{}

==> tikz-quadratic-bipartite-matching-strategy.tex <==
\piDeclareString{job}{}
\piDeclareBool{beamer}{true}
\piDeclareBool{debug}{false}
\piDeclareBool{main graph}{false}
\piDeclareBool{auxiliary graph}{false}
\piDeclareBool{hat point}{false}
\piDeclareBool{bar point}{false}
\piDeclareBool{bar matchings}{false}
\piDeclareBool{convex combination}{false}
\piDeclareBool{bar matchings structure}{false}
\piDeclareBool{hat matchings}{false}
\piDeclareBool{hat matchings portion}{false}
\piDeclareBool{hat matchings barycenter}{false}

\piParse % Parses all given options

% Debugging code

\def\boundingbox{(-5.8,-3.5) rectangle (5.8,3.6)};

\draw[clip,use as bounding box,draw=none] \boundingbox;

\piIfBool{debug}{
  \draw[step=.5cm,help lines] (-11,-20) grid (11,20);
  \draw[draw=red,thick] \boundingbox;
}{}

\piIfBool{main graph}{
  \piIfBool{auxiliary graph}{
    \draw[dashed,black!50!white] (0,-3.5) -- (0,3.7);
  }{}

  \node[anchor=east] at (-0.1,3.3) {Graph $K_{m,n}$};  
}{}

\piIfBool{hat point}{
  \node[draw=black, thick, rectangle, rounded corners] (upper left) at (-3.5,2) {%
    \begin{minipage}{42mm}
      \begin{center}
        $(\hat{x},\hat{y})$ satisfies a certain \\
        inequality with equality.
      \end{center}
    \end{minipage}};
}{}

\piIfBool{auxiliary graph}{
  \node[anchor=west] at (0.1,3.3) {Related graph $\bar{G}$};
}{}


\piIfBool{bar point}{
  \node[draw=black, thick, rectangle, rounded corners] (upper right) at (3.5,2) {%
    \begin{minipage}{42mm}
      \begin{center}
        Vector $\bar{x}$ in certain face ($\blackdiamond$) \\
        of $\bar{G}$'s matching polytope.
      \end{center}
    \end{minipage}}; 

  \piIfBool{hat point}{
    \draw[very thick,->] (upper left) to node[above] {construct} (upper right);
  }{}
}{}

\piIfBool{bar matchings}{
  \node[draw=black, thick, rectangle, rounded corners] (lower right) at (3.5,-2) {%
    \begin{minipage}{42mm}
      \begin{center}
        Matchings $\bar{M}_1,\ldots,\bar{M}_k$ \\
        in $\bar{G}$.
      \end{center}
    \end{minipage}};
    
  \piIfBool{bar point}{
  \draw[very thick,->] (upper right) to node[above, rotate=90] {exists} node[right=2mm] {%
    \begin{minipage}{22mm}
      \piIfBool{convex combination}{
        Convex \\
        combination \\
        with special \\
        property ($\bigstar$)
      }{}
    \end{minipage}} (lower right);
  }{}
}{}

\piIfBool{bar matchings structure}{
  \node at (3.5,-3) {%
    \begin{minipage}{33mm}
      $\bar{M}_j$ have structure \\
      due to ($\blackdiamond$) and ($\bigstar$).
    \end{minipage}};
}{}

\piIfBool{hat matchings}{
  \node[draw=black, thick, rectangle, rounded corners] (lower left) at (-3.5,-2) {%
    \begin{minipage}{42mm}
      \begin{center}
        Matchings $\hat{M}_1,\ldots,\hat{M}_k$ \\
        in $K_{m,n}$.
      \end{center}
    \end{minipage}};
    
  \piIfBool{bar matchings}{
    \draw[very thick,->] (lower right) to node[above] {construct} (lower left);
  }{}
}{}

\piIfBool{hat matchings portion}{
  \node at (-3.5,-3) {%
    \begin{minipage}{33mm}
      $\hat{y}k$ of them contain \\
      the edges $e_1$ and $e_2$.
    \end{minipage}};
}{}

\piIfBool{hat matchings barycenter}{
  \draw[very thick,->] (lower left) to node[rotate=90,above] {prove} node[right=2mm] {%
    \begin{minipage}{20mm}
      Barycenter \\
      of all $\chi(\hat{M}_j)$ \\
      is equal to $\hat{x}$.
    \end{minipage}} (-3.5,1.0);
}{}

